Transverse momentum distributions in low-mass Drell-Yan lepton pair production at NNLO QCD

The production of lepton pairs at low invariant mass and finite transverse momentum resolves QCD dynamics at the boundary between the perturbative and non-perturbative domains. We investigate the impact of NNLO QCD corrections on these observables at energies corresponding to the BNL RHIC collider and to fixed-target experiments. Satisfactory perturbative convergence is observed in both cases. Only the collider data are found to be well-described by perturbative QCD, thus indicating the importance of non-perturbative effects in lepton-pair transverse momentum distributions at fixed target energies.

==> fig.tex <==
% Some definitions
\makeatletter

\newif\ifstartcompletesineup
\newif\ifendcompletesineup
\pgfkeys{
    /pgf/decoration/.cd,
    start up/.is if=startcompletesineup,
    start up=true,
    start up/.default=true,
    start down/.style={/pgf/decoration/start up=false},
    end up/.is if=endcompletesineup,
    end up=true,
    end up/.default=true,
    end down/.style={/pgf/decoration/end up=false}
}
\pgfdeclaredecoration{complete sines}{initial}
{
    \state{initial}[
        width=+0pt,
        next state=upsine,
        persistent precomputation={
            \ifstartcompletesineup
                \pgfkeys{/pgf/decoration automaton/next state=upsine}
                \ifendcompletesineup
                    \pgfmathsetmacro\matchinglength{
                        0.5*\pgfdecoratedinputsegmentlength / (ceil(0.5* \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) )
                    }
                \else
                    \pgfmathsetmacro\matchinglength{
                        0.5 * \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) - 0.499)
                    }
                \fi
            \else
                \pgfkeys{/pgf/decoration automaton/next state=downsine}
                \ifendcompletesineup
                    \pgfmathsetmacro\matchinglength{
                        0.5* \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) - 0.4999)
                    }
                \else
                    \pgfmathsetmacro\matchinglength{
                        0.5 * \pgfdecoratedinputsegmentlength / (ceil(0.5 * \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength ) )
                    }
                \fi
            \fi
            \setlength{\pgfdecorationsegmentlength}{\matchinglength pt}
        }] {}
    \state{downsine}[width=\pgfdecorationsegmentlength,next state=upsine]{
        \pgfpathsine{\pgfpoint{0.5\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}
        \pgfpathcosine{\pgfpoint{0.5\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}
    }
    \state{upsine}[width=\pgfdecorationsegmentlength,next state=downsine]{
        \pgfpathsine{\pgfpoint{0.5\pgfdecorationsegmentlength}{-0.5\pgfdecorationsegmentamplitude}}
        \pgfpathcosine{\pgfpoint{0.5\pgfdecorationsegmentlength}{0.5\pgfdecorationsegmentamplitude}}
}
    \state{final}{}
}


\pgfdeclaredecoration{spring}{initial}
{
  \state{initial}[
    width=+0pt,
    next state=coil,
    persistent precomputation={
      \pgfmathsetmacro\matchinglength{
        (ceil(\pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) - \pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) > 0.5
        ? (\pgfdecoratedinputsegmentlength - 2 * \pgfdecorationsegmentaspect * \pgfdecorationsegmentamplitude) / (floor(\pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) + 0.499)
        : (\pgfdecoratedinputsegmentlength - 2 * \pgfdecorationsegmentaspect * \pgfdecorationsegmentamplitude) / (ceil(\pgfdecoratedinputsegmentlength / \pgfdecorationsegmentlength) + 0.499)
      }
      \setlength{\pgfdecorationsegmentlength}{\matchinglength pt}
    },
  ]{}
  \state{coil}[
    switch if less than=%
      0.5\pgfdecorationsegmentlength%
      +\pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude%
      +\pgfdecorationsegmentaspect\pgfdecorationsegmentamplitude to last,
    width=+\pgfdecorationsegmentlength,
  ]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{ 1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{ 2}}
    {\pgfpoint@oncoil{1    }{ 1    }{ 3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{ 4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{ 5}}
    {\pgfpoint@oncoil{2    }{ 0    }{ 6}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{2    }{-0.555}{ 7}}
    {\pgfpoint@oncoil{1.555}{-1    }{ 8}}
    {\pgfpoint@oncoil{1    }{-1    }{ 9}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{0.445}{-1    }{10}}
    {\pgfpoint@oncoil{0    }{-0.555}{11}}
    {\pgfpoint@oncoil{0    }{ 0    }{12}}
  }
  \state{last}[next state=final]
  {
    \pgfpathcurveto
    {\pgfpoint@oncoil{0    }{ 0.555}{1}}
    {\pgfpoint@oncoil{0.445}{ 1    }{2}}
    {\pgfpoint@oncoil{1    }{ 1    }{3}}
    \pgfpathcurveto
    {\pgfpoint@oncoil{1.555}{ 1    }{4}}
    {\pgfpoint@oncoil{2    }{ 0.555}{5}}
    {\pgfpoint@oncoil{2    }{ 0    }{6}}
  }
  \state{final}{}
}



\tikzset{
      % style to apply some styles to each segment of a path
      on each segment/.style={
        decorate,
        decoration={
          show path construction,
          moveto code={
          },
          lineto code={
            \path [#1]
            (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          },
          curveto code={
            \path [#1] (\tikzinputsegmentfirst)
            .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..
            (\tikzinputsegmentlast);
          },
          closepath code={
            \path [#1]
            (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          },
        },
      },
    % vector (old)
    vector/.style={line join=round, line cap=round, line width=0.1+0.02*\tikz@node@distance, decorate, decoration={complete sines, segment length=0.15*\tikz@node@distance, amplitude=0.2*\tikz@node@distance, start up}},
    % vector2 (old)
    vector2/.style={line join=round, line cap=round, line width=0.1+0.02*\tikz@node@distance, decorate, decoration={complete sines, segment length=0.15*\tikz@node@distance, amplitude=0.2*\tikz@node@distance, start down}},
    % gluon (old)
    gluon/.style={line join=round, line cap=round, line width=0.1+#1*0.02*\tikz@node@distance, decorate, decoration={spring, amplitude=#1*0.1*\tikz@node@distance, segment length=#1*0.18*\tikz@node@distance, aspect=#1*0.66}},
    gluon/.default=1.0,
    % Quark style: scalable arrowheads (properly centered)
    quark/.style args={#1}{
        line join=round,
        line cap=round,
        line width=0.1+0.02*\tikz@node@distance,
        postaction={
            on each segment={
                decorate,
                decoration={
                    markings,
                    % position = midpath + half of arrowhead length
                    mark=at position (0.5*\pgfdecoratedpathlength+0.08*#1*\tikz@node@distance) with
                    \arrow{Stealth[length={#1*0.16*\tikz@node@distance}, width={#1*0.14*\tikz@node@distance}]}
                }
            }
        }
    },
    quark/.default={1.0},
    % Top quark (thick quark, default arrowheads are 1.2x quark)
    tquark/.style={quark={#1}, line width=0.1+0.06*\tikz@node@distance},
    tquark/.default={1.2},
    % Quark line without arrowheads
    qline/.style={line join=round, line cap=round, line width=0.1+0.02*\tikz@node@distance},
    % Higgs line
    higgs/.style={line join=round, line cap=round, line width=0.1+0.02*\tikz@node@distance, dashed}
}

\newcommand\myaction{}



% VHJ Feynman diagrams

% Top loop RRI VHJ (OpenLoops has it, we cannot: corresponing VV are unknown)
\newcommand{\TopRRI}[2][0]{\tikz[node distance=#2, baseline=#1]
    {
        \draw [quark] (0,0) -- ++(0:#2) coordinate (qV) -- ++(-90:0.75*#2) coordinate (qg1) -- ++(-90:0.75*#2) coordinate (qg2) -- ++(180:#2);
        \draw [vector] (qV) -- ++(0:0.85*#2) coordinate (Vl);
        \draw [gluon] (qg2) -- ++(0:0.85*#2) coordinate (g1t);
        \draw [gluon] (qg1) -- ++(0:0.85*#2);
        \draw [tquark] (g1t) -- ++(30:#2) coordinate (g2t) -- ++(-90:#2) coordinate (Ht) -- (g1t);
        \draw [gluon] (g2t) -- ++(0:#2);
        \draw [higgs] (Ht) -- ++(0:#2);
        \draw [quark] (Vl)++(30:0.75*#2) -- (Vl) -- ++(-30:0.75*#2);
        \coordinate (label) at ($(g1t)+({sqrt(3)/4*#2},0)$);
        \node[xshift=0.12*#2] at (label) {$\Pqt$};
    }
}


% Genuine (only Yukawa) two-loop correction to VHJ
\newcommand{\TopRVI}[2][0]{\tikz[node distance=#2, baseline=#1]
    {
        \draw [quark] (0,0) -- ++(0:#2) coordinate (qV) -- ++(-90:#2) coordinate (qg1) -- ++(-90:#2) coordinate (qg2) -- ++(180:#2);
        \draw [gluon] (qg1) -- ++(0:#2) coordinate (tg1);
        \draw [gluon] (qg2) -- ++(0:#2) coordinate (tg2);
        \draw [tquark] (tg2) -- (tg1) -- ++(0:#2) coordinate (tg3) -- ++(-90:#2) coordinate (tH) -- cycle;
        \draw [gluon] (tg3) -- ++(0:#2);
        \draw [higgs] (tH) -- ++(0:#2);
        \draw [vector] (qV) -- ++(0:#2) coordinate (Vl);
        \draw [quark] (Vl)++(30:0.75*#2) -- (Vl) -- ++(-30:0.75*#2);
        \coordinate (label) at ($(tg1)!0.5!(tH)$);
        \node at (label) {$\Pqt$};
    }
}


% VHJ Top loop Yukawa-induced (box, included)
\newcommand{\TopZHJI}[2][0]{\tikz[node distance=#2, baseline=#1]
    {
        \draw [gluon] (0,0) -- ++(0:#2) coordinate (g1t);
        \draw [tquark] (g1t) -- ++(18:#2) coordinate (tV) -- ++(-54:#2) coordinate (tH) -- ++(-126:#2) coordinate (g2t) -- ++(-198:#2) coordinate (g3t) -- cycle;
        \draw [gluon] (g2t) -- ++(0:#2);
        \draw [gluon] (g3t) -- ++(0:-#2);
        \draw [vector2] (tV) -- ++(0:0.85*#2) coordinate (Vl);
        \draw [higgs] (tH) -- ++(0:#2);
        \draw [quark] (Vl)++(30:0.75*#2) -- (Vl) -- ++(-30:0.75*#2);
        \coordinate (mid) at ($(g3t)!0.5!(g1t)$);
        \coordinate (label) at ($(mid)!0.5!(tH)$);
        \node [xshift=-0.05*#2] at (label) {$\Pqt$};
    }
}


% VHJ Top loop Drell--Yan-like (triangle, included)
\newcommand{\TopZHJII}[2][0]{\tikz[node distance=#2, baseline=#1]
    {
        \draw [gluon] (0,0) -- ++(0:#2) coordinate (gt1);
        \draw [tquark] (gt1) -- ++(0:#2) coordinate (tV) -- ++(-90:#2) coordinate (gt2) -- ++(-180:#2) coordinate (gt3) -- cycle;
        \draw [gluon] (gt2) -- ++(0:#2);
        \draw [gluon] (gt3) -- ++(0:-#2);
        \draw [vector] (tV) -- ++(0:0.75*#2) coordinate (VH);
        \draw [vector] (VH) -- ++(45:0.75*#2) coordinate (Vl);
        \draw [higgs] (VH) -- ++(-45:#2);
        \draw [quark] (Vl)++(75:0.75*#2) -- (Vl) -- ++(15:0.75*#2);
        \coordinate (label) at ($(tV)!0.5!(gt3)$);
        \node at (label) {$\Pqt/\Pqb$};
    }
}


\newcommand{\VHJrrB}[4][0]{\tikz[node distance=#4, baseline=#1]
    {
    \draw [quark] (0,0) -- ++(0:#4) coordinate (qg1) -- ++(-90:1.5*#4) coordinate (qV) -- ++(-180:#4);
    \draw [vector] (qV) -- ++(0:0.75*#4) coordinate (VH);
    \draw [vector] (VH) -- ++(30:0.85*#4) coordinate (Vl);
    \draw [higgs] (VH) -- ++(-30:{(0.85+cos(22.5)*0.75)*#4});
    \draw [quark] (Vl)++(52.5:0.75*#4) -- (Vl) -- ++(7.5:0.75*#4);
    \path (qg1)++(-90:0.5*#4) coordinate (qg2);
    \path (qg2)++(-90:0.5*#4) coordinate (qg3);

    % Draw gluon radiation if 1 < #2
    \path \pgfextra{\ifthenelse{0 < #2}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qg1) -- ++(15:#4);

    % Draw second gluon radiation if 1 < #2
    \path \pgfextra{\ifthenelse{0 < #2}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qg3) -- ++(15:#4);

    % Draw gluon radiation if 2 < #2
    \path \pgfextra{\ifthenelse{1 < #2}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qg2) -- ++(15:#4);


    % Draw gluon loop if 0 < #3
    \path (qV)++(-180:0.7*#4) coordinate (qgl);
    \path (qg2)++(90:0.1*#4) coordinate (qgl2);
    \path \pgfextra{\ifthenelse{0 < #3}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qgl2) to [bend right=45] (qgl);

    % Draw another one if 1 < #3 (manual adjustions, duh...)
    \path \pgfextra{\ifthenelse{1 < #3}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (qg3)++(-90:0.16*#4) arc (-90:0:0.56*#4) coordinate (new);
    \path \pgfextra{\ifthenelse{1 < #3}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (new) arc (0:90:0.56*#4);
    \path \pgfextra{\ifthenelse{1 < #3}{\renewcommand\myaction{draw}}{}} [gluon,\myaction] (new)++(15:#4) -- ($(new)+(-10:0.03*#4)$);

    }
}

